Concurrent self-adjusting distributed tree networks

SplayNets are a distributed generalization of the classic splay tree data structures. Given a set of communication requests and a network comprised of n nodes, such that any pair of nodes is capable of establishing a direct connection, the goal is to dynamically find a (locally routable) binary tree topology, which connects all nodes and optimizes the routing cost for that communication pattern, making local topology transformations (rotations) before each request is served. In this work we present a distributed and concurrent implementation of SplayNets. Analytical results show that our proposed algorithm prevents loops and deadlocks from occurring between concurrent rotations. We compute the total amortized average cost of a splay request in number of rounds and number of time-slots and as a function of the empirical entropies of source and destination nodes of the splay requests.

==> abstract.tex <==
\begin{abstract}
SplayNets are a distributed generalization of the classic splay tree data structures. Given a set of communication requests and a network comprised of $n$ nodes, such that any pair of nodes is capable of establishing a direct connection, the goal is to dynamically find and adjust a (locally routable) tree topology which optimizes the routing cost for the given communication pattern and minimizes the topological reconfiguration costs. We present the first concurrent implementation of such self-adjusting SplayNets. Analytical results show that our proposed algorithm prevents loops and deadlocks from occurring between concurrent rotations. We compute the total amortized average cost of a splay request in number of rounds and number of time-slots and as a function of the empirical entropies of source and destination nodes of the splay requests. 

\end{abstract}
\keywords{Distributed data structures, splay trees, concurrency, routing, SplayNets}

==> resumo.tex <==
%\begin{abstract}
SplayNets s\~ao uma generaliza\c c\~ao distribu\'ida da estrutura de dados cl\'assica splay tree. Dado um conjunto de requisi\c c\~oes de comunica\c c\~ao e uma rede composta de $n$ n\'os, tal que qualquer par de n\'os \'e capaz de estabelecer uma conex\~ao direta, o objetivo \'e encontrar uma topologia de \'arvore bin\'aria dinamicamente, que conecta todos os n\'os e otimiza o custo de roteamento para o padr\~ao de comunica\c c\~ao, realizando transforma\c c\~oes de topologia locais (rota\c c\~oes) antes de servir qualquer requisi\c c\~ao. Neste trabalho, apresentamos uma implementa\c c\~ao distribu\'ida e concorrente das SplayNets. Resultados anal\'iticos mostram que nosso algoritmo proposto impede a ocorr\^encia de loops e deadlocks entre rota\c c\~oes concorrentes. N\'os calculamos o custo  m\'edio amortizado total de uma requisi\c c\~ao de splay em n\'umeros de rounds e n\'umero de intervalos de tempo (time-slots) e como uma fun\c c\~ao da entropia emp\'irica dos n\'os fonte e destino de uma requisi\c c\~ao de splay. 

%\end{abstract}
\keywords{Estruturas de dados distribu\'idas, splay trees, concorr\^encia, roteamento, SplayNets}
